On Graph Neural Networks versus Graph-Augmented MLPs

From the perspective of expressive power, this work compares multi-layer Graph Neural Networks (GNNs) with a simplified alternative that we call Graph-Augmented Multi-Layer Perceptrons (GA-MLPs), which first augments node features with certain multi-hop operators on the graph and then applies an MLP in a node-wise fashion. From the perspective of graph isomorphism testing, we show both theoretically and numerically that GA-MLPs with suitable operators can distinguish almost all non-isomorphic graphs, just like the Weifeiler-Lehman (WL) test. However, by viewing them as node-level functions and examining the equivalence classes they induce on rooted graphs, we prove a separation in expressive power between GA-MLPs and GNNs that grows exponentially in depth. In particular, unlike GNNs, GA-MLPs are unable to count the number of attributed walks. We also demonstrate via community detection experiments that GA-MLPs can be limited by their choice of operator family, as compared to GNNs with higher flexibility in learning.

==> draft_v0.tex <==
% \documentclass{article}
\usepackage{tgpagella}
\usepackage[utf8]{inputenc}
\usepackage[dvips,letterpaper,margin=1.2in]{geometry}
\usepackage[square,sort,comma,numbers]{natbib}
\usepackage{amsmath}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{natbib}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{graphicx}

\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

\title{Shallow Graph Neural Networks with Multi-hop Operators: Expressive Power and Learning}

% \title{multi-hop vs depth}
% \author{zc1216 }
% \date{August 2020}

\begin{document}

\maketitle

Outline:
\begin{enumerate}
    \item Expressive power from the view point of graph isomorphism testing
    \begin{itemize}
        \item (Theory) Negative example for the case $\Omega = \{ A, A^2, ... \}$
        \item (Theory) Can distinguish almost all random graphs if $AD^{-\alpha} \in \Omega$ for large enough $\alpha$
        \item (Numerics) Number of graph-equivalent-classes on real datasets - Simplified GNN $\simeq$ GNN
    \end{itemize}
    \item Expressive power from the view point of approximating node functions
    \begin{itemize}
        \item (Numerics) Number of node-equivalent-classes on real datasets - Simplified GNN $<$ GNN
        \item (Theory) GNN induces double-exponentially-in-depth many node-equivalence-classes
        \item (Theory) With $\Omega$ being powers of normalized adjacency, Simplified GNN induces exponential-of-polynomial-of-depth
        \item (Theory) For any $\Omega$, there exists a node-equivalence-class induced by this Simplified GNN that contains double-exponentially-in-depth many rooted subtrees.
        \item (Theory) For any $\Omega$, Simplified GNN cannot count any specific walk on all graphs.
        \item (Uncertain)(Experiment) Fitting random functions on random regular graphs.
    \end{itemize}
    \item Generalization
    \begin{itemize}
        \item (Theory) VC dimension comparison of GNNs and Simplified GNNs (with $\Omega$ being powers of normalized adjacency) from the above results 
        \item (Uncertain)(Theory) Transductive generalization bounds based on the VC dimension.
    \end{itemize}
    \item NTK limit
\end{enumerate}

\section{Introduction}
Motivations for using multi-hop operators instead of adding depth:
\begin{itemize}
    \item Scalability
    \item Optimization - exploding and vanishing gradients
\end{itemize}
Main questions: by using multi-hop operators instead of adding depth,
\begin{itemize}
    \item (How) is expressive power sacrificed? 
    \item Do we gain in generalization?
\end{itemize}
\section{Background}


\subsection{Model}
Consider a graph $G = (V, E)$ with node features denoted by $X \in \mathbb{R}^{n \times d}$ and no edge features. Let $\Omega(A) = \{ \omega_1(A)$, ..., $\omega_T(A) \}$ be a set of (usually multi-hop) operators that are functions of the adjacency matrix, $A$. In its most general form, such a model first computes a series of augmented features through operators in $\Omega(A)$ 
\begin{equation}
\label{eq:update_1}
    \tilde{X}_t = \omega_t(A) \cdot \phi_t(X)
\end{equation}
with $\phi_t: \mathbb{R}^d \to \mathbb{R}^{\tilde{d}}$ being a learnable function acting as a feature transformation applied to each node separately, and can be realized by an MLP. Next, the model 
concatenates $\tilde{X}_1, ..., \tilde{X}_T$ into $\tilde{X} = [\tilde{X}_1, ..., \tilde{X}_T] \in \mathbb{R}^{n \times (T \tilde{d})}$, and compute
\begin{equation}
\label{eq:update_2}
    Z = \rho(\tilde{X})~,
\end{equation}
where $\rho: \mathbb{R}^{T \tilde{d}} \to \mathbb{R}^{d'}$ is also a learnable node-wise function, usually realized by an MLP, $\rho(Y) = \sigma(Y W_1) W_2$. 

Within this general form, we mention two particular variants: In the first variant, we do not concatenate the augmented features but rather sum them, that is replacing \eqref{eq:update_2} by
\begin{equation}
    Z = \rho(\sum_{t=1}^T \tilde{X}_t)~,
\end{equation}
We will show later that when $\phi_t$ and $\rho$ are expressive enough, this variant attains the level of expressive power of the general model. A second variant motivated by computational efficiency is to replace each $\phi_t$ by a linear function, in which case \eqref{eq:update_1} can be written as
\begin{equation}
    \tilde{X}_t = \omega_t(A) \cdot X \cdot \Theta_t~,
\end{equation}
with $\Theta_t \in \mathbb{R}^{d \times \tilde{d}}$. Such a choice is advantageous in terms of computational efficiency since the matrix product $\omega_t(A) \cdot X$ can be pre-computed before training \cite{rossi2020sign}. We will also show later that this simplification does not lose expressive power in the case if the node features are identical.


% computes
% \begin{equation}
%     Z = \rho(\sum_{t=1}^T \omega_t(A) \cdot \tilde{X}_t)~,
% \end{equation}
% where $\rho: \mathbb{R}^{\tilde{d}} \to \mathbb{R}^{d'}$ is also a node-wise function, usually realized by an MLP, $\rho(Y) = \sigma(Y W_1) W_2$.
\subsection{Some examples}
% Here are some examples:
\begin{itemize}
    \item Simple Graph Convolution \cite{wu2020simplifying}:\\
    $\Omega(A) = \{ (\tilde{D}^{-1/2} \tilde{A} \tilde{D}^{-1/2})^T \}$ for some $T > 0$, with $\tilde{A} = A + I$ and $\tilde{D}$ being the degree matrix of $\tilde{A}$; 
    % $\sigma$ being the softmax function.
    $\rho(H) = softmax(H W)$. Thus,
    \begin{equation}
        \hat{Y} = \phi(softmax((\tilde{D}^{-1/2} \tilde{A} \tilde{D}^{-1/2})^T X W))
    \end{equation}
    
    \item Graph Feature Network \cite{chen2019powerful}:\\
    $\Omega(A) = \{ I, D, \omega_1(A)$, ..., $\omega_T(A) \}$, with $\omega_t(A) = (\tilde{D}^{-1/2} (A + \epsilon I) \tilde{D}^{-1/2})^t$; $\rho$ is an MLP applied to the vectorization of $Z_{i, :, :} \in \mathbb{R}^{T \times d_0}$ for each node $i$; $\phi$ is also an MLP.
    
    \item Scalable Inception Graph Networks \cite{rossi2020sign}:\\
    $\Omega(A) = \Omega_1(A) \cup \Omega_2(A) \cup \Omega_3(A)$, where $\Omega_1(A)$ is a family of simple / normalized adjacency matrices, $\Omega_2(A)$ is a family of Personalized-PageRank-based adjacency matrices, and $\Omega_3(A)$ is a family of ``triangle-based" adjacency matrices; $\rho: \mathbb{R}^{n \times d_0 \times T} \to \mathbb{R}^{n \times Td_1}$, defined to be 
    $\rho(Z)_{:, :, (t-1)d_1:td_1} = \sigma_2(\sigma_1(Z_{:, :, t} W_t)W_{out})$ with each $W_t \in \mathbb{R}^{d_0 \times d_1}$ and $W_{out} \in \mathbb{R}^{T d_1 \to d'}$.
    
\end{itemize}

\section{Expressive Power as Graph Isomorphism Tests}
We first study the expressive power of Simplified GNNs via their ability to distinguish nonisomorphic graphs. It is shown in \cite{xu2018powerful, morris2019higher} that GNNs based on neighborhood-aggregation are no more powerful than the Weisfeiler-Lehman (WL) test, in the sense that for any pair of graphs that cannot be distinguished by the WL test, any such GNN will return the same output when applied to them. A natural question to ask is, by replacing the network depth with multi-hop operators, do Simplified GNNs sacrifice the ability to distinguish certain pairs of graphs? We first give an example where a concrete example can be found:
% Consider the choice of $\Omega(A) = \{ A, ..., A^K\}$.
% \begin{proposition}
% Such a model is as powerful as the following test of graph isomorphism:\\
% \textbf{Simplified WL-1 (SWL-1):} Define $w_t(i, j)$ to be the number of walks (allowing backtracking) of length t from $i$ to $j$. For $t \in \{1, …, T\}$,
% \begin{align}
%     \tilde{c}^{t}(i) =& \cup_{count \leq w_t(i, j)} \{\{ c^{0}(j) \}\}_{j \in N_1(i)} \\
% c^{out}(i) =& (c^{0}(i), \tilde{c}^{1}(i), …, \tilde{c}^{T}(i))
% \end{align}
% \end{proposition}
\begin{proposition}
If either $\Omega \subseteq \{ AD^{-1}, (AD^{-1})^2, ..., (AD^{-1})^T, ...\}$ or $\Omega \subseteq \{ A, A^2, ..., A^T, ...\}$, then there exist a pair of graphs which can be distinguished by the WL test but not such a Simplified GNN.
\end{proposition}

% First, it is not hard to see that the power of SWL-1 in distinguishing non-isomorphic graphs is no greater than that of WL. In fact, the inequality is strict:

% \begin{proposition}
% There exists a pair of graph that can be distinguished by $2$ iterations of WL but not by any iterations of SWL-1.
% \end{proposition}

Nonetheless, we next show that if we focus on not particular counterexamples but rather the averaged performance in distinguishing random graphs, it is not hard for Simplified GNNs to reach the same level as WL, which is known to distinguish almost all pairs of random graphs under a uniform distribution \cite{babai1980random}. Specifically, we have
% if we look at the average performance on random graphs rather than the adversarial examples, the power of SWL-1 is decent:
% From \cite{babai1980random}, we have
% \begin{lemma}
% Two iterations of WL is able to distinguish ``almost all" random graphs.
% \end{lemma}
% Therefore, since SWL-1 can express two iterations of 
% \begin{proposition}
% Two iterations of Simplified WL-1 is able to distinguish ``almost all" random graphs.
% \end{proposition}
\begin{proposition}
Consider graphs with node degrees upper-bounded by $\bar{d}$. If $A D^{-\alpha} \in \Omega$ for some $\alpha > (1 - \log_{\bar{d}}(\bar{d}-1))^{-1}$, then the Simplified GNN is able to distinguish almost all pairs of random graphs under the uniform distribution.  
\end{proposition}

% Hence, in this regard, SWL-1 is expressive enough in terms of graph isomorphism testing. But from another view, this suggests that graph isomorphism testing may not be the best perspective for comparing the expressive power of GNN models. We propose an alternative in the next section.

We supplement this theoretical result with the following calculations on real datasets. Given a space of graphs and a family $\mathcal{F}$ of functions mapping $\mathcal{G}$ to $\mathbb{R}$, $\mathcal{F}$ induced an equivalence relation $\simeq_{\mathcal{G}; \mathcal{F}}$ among graphs in $G$ such that for $G_1, G_2 \in \mathcal{G}$, $G_1 \simeq_{\mathcal{G}; \mathcal{F}} G_2$ if and only if $\forall f \in \mathcal{F}$, $f(G_1) = f(G_2)$. For example, if $\mathcal{F}$ is powerful enough to distinguish all pairs of non-isomorphic graphs, then each equivalence class under $\simeq_{\mathcal{G}, \mathcal{F}}$ contains exactly one graph. Thus, by looking at the number or sizes of the equivalence classes induced by different families of functions on $\mathcal{G}$, we can evaluate their relative expressive power in a quantitative way. We see from the table that indeed, both GNN and Simplified GNN achieve a decent level of power measured on real datasets. 

\subsection{Enhancing the power with additional operators}
Consider another choice of $\Omega(A) = \{ \min(A, 1), ..., \min(A^K, 1)\}$.
\begin{proposition}
Such a model is as powerful as the following test of graph isomorphism:\\
\textbf{Simplified WL-2 (SWL-2):}
For $t \in \{1, …, T\}$,
\begin{align}
    \tilde{c}^{t}(i) =& \cup_{j \in N_t(i)} \{\{ c^{0}(j) \}\} \\
c^{out}(i) =&(c^{0}(i)), \tilde{c}^{1}(i), …, \tilde{c}^{T}(i))
\end{align}
\end{proposition}
\begin{proposition}
SWL-2 is able to count triangles.
\end{proposition}
\begin{corollary}
There exists pairs of graphs that can be distinguished by SWL-2 but not by SWL-1 or WL.
\end{corollary}


\section{Expressive Power in Representing Node-wise Functions on Rooted Subtrees}
To study the expressive power of GNN models in a more fine-grained way, we consider the setting of node-wise prediction tasks. In these tasks, whether supervised or semi-supervised, the goal can be considered as fitting a real-valued function which takes a graph and a node index as its input, i.e., mapping a graph $G$ together with a node $i$ in $G$ to $f(G, i) \in \mathbb{R}$.
% which takes as its input the local neighborhood of the node in the graph, and outputs the desired label for the node. 
We are particularly interested in local algorithms, including GNNs based on message passing as well as Simplified GNNs with multi-hop operators, which only takes advantage of the information in a $k$-hop neighborhood of $i$ in $G$ for some $k > 0$. Thus, such a model defines a function on the space of depth-$k$ egonets \cite{preciado2010local}, which we denote by $\mathcal{G}^{[\texttt{ego}, k]}$. Note that an egonet of depth-$k$ can be equivalently represented by a graph-node pair, where the graph has diameter at most $k$ and the node indicates the root of the egonet.
% We next study the expressiveness of GNNs and Simplified GNNs as families of such functions.

To study the expressiveness of GNNs and Simplified GNNs as families of such functions, we introduce a different set of equivalence relations induced on the space of depth-$k$ egonets. Assuming that the node features are discrete, given a family of functions $\mathcal{F}$ on $\mathcal{G}^{[\texttt{ego}, k]}$, we can define an equivalence relation $\simeq_{\mathcal{G}^{[\texttt{ego}, k]}; \mathcal{F}}$ among depth-$k$ egonets such that $\forall G_1, G_2 \in \mathcal{G}^{[\texttt{ego}, k]}$, $G_1 \simeq_{\mathcal{G}^{[\texttt{ego}, k]}; \mathcal{F}} G_2$ if and only if $\forall f \in \mathcal{F}$, $f(G_1) = f(G_2)$. By looking at the number or sizes of these induced equivalence classes, we can evaluate the relative expressive power of different families of functions on depth-$k$ egonets in a quantitative way. 

First, since the WL test only takes into account the rooted subtree information in distinguishing neighborhoods, each equivalence class induced by WL-type GNNs consists of all depth-$k$ egonets that give rise to the same depth-$k$ rooted subtree. Thus, to count the number of node equivalence classes induced by WL-type GNNs, we first count the number of computation trees.
In what follows, consider the case where node features are binary and all nodes have degree at most $m$. 
% Let $\mathcal{T}^{(k, m)}$ be the space of all computation trees (rooted subtrees) of depth $k$ and degree at most $m$, in which each node has feature $0$ or $1$.
Let $\mathcal{T}^{(k, m)}$ be the space of all computation trees (rooted subtrees) of depth $k$ and degree at most $m$, in which each node has feature $0$ or $1$.
\begin{lemma}
$|\mathcal{T}^{(k, m)}| \geq (m-1)^{(2^{k}-1)}$.
\end{lemma}
\begin{proof}
let $L^{(k)}(T)$ denote the set of the depth-$k$ leaf nodes of a tree $T$. There are $2^k$ paths of length $k$, from $(0, 0, ..., 0)$ to $(1, 1, ..., 1)$. We index them according to the dictionary order, with $\mathtt{P}^{(k)}_1 = (0, 0, ..., 0)$ and $\mathtt{P}^{(k)}_{2^k} = (1, 1, ..., 1)$.
To lower-bound the cardinality of $\mathcal{T}^{(k, m)}$, we lower-bound the cardinality of its subset, $\tilde{\mathcal{T}}^{(k, m)}$, defined to be those computation trees in $\mathcal{T}^{(k, m)}$ which contain all $2^k$ possible paths of length $k$. This means that, for each $T \in \tilde{\mathcal{T}}^{(k, m)}$, $L^{(k)}(T) = \cup_{\tau = 1}^{2^k} S_{\tau}$, with each $S_{\tau}$ non-empty and satisfying that the path from the root node to every node in $S_{\tau}$ is exactly $\mathtt{P}^{(k)}_\tau$.

% $\exists$ nodes $i_1^{(k, m)}, ..., i_{2^k}^{(k, m)}$ such that the paths from the root node to each of them are all distinct. 
Next, we construct computation trees of depth $k+1$ by assigning children of feature $0$ or $1$ to the leaf nodes in $T$. First note that, with two distinct computation trees $T$ and $T' \in \tilde{\mathcal{T}}^{(k, m)}$, we obtain distinct computation trees in $\tilde{\mathcal{T}}^{(k+1, m)}$ in this way. There are obviously many choices to assign the children. To get a lower-bound on the cardinality of $\tilde{\mathcal{T}}^{(k+1, m)}$, we only need to consider a subset of these choices of assignments, namely, those that assign the same number of children with feature $1$ to nodes in the same $S_{\tau}$.
Thus, we let $\bar{m}_\tau$ denote the number of children of feature $1$ assigned to the nodes in $S_\tau$. Due to the constraint that each node in the computation subtree must have its parent's feature as one of its children's feature, not all choices of $\{ \bar{m}_\tau \}_{\tau=1}^{2^k}$ lead to legitimate computation trees. Nonetheless, when restricting to the cases where $\forall \tau \in [2^k], 1 \leq \bar{m}_{\tau} \leq m-1$, we see that every node in $L^{(k)}(T)$ has at least one child of feature $0$ and another child of feature $1$, thereby satisfying the constraint whether its parent has feature $0$ or $1$. Moreover, because of this, the new tree of depth $k+1$ obtained in this way contains all $2^{k+1}$ possible paths of length $k+1$, and therefore belongs to $\tilde{\mathcal{T}}^{(k+1, m)}$. Hence, what is left to do is to show a lower bound on how many such trees in $\tilde{\mathcal{T}}^{(k+1, m)}$ can be obtained from each $T$. Because nodes in $S_\tau$ are distinguishable from nodes in $S_{\tau'}$ for $\tau \neq \tau'$, we see that every choice of the $2^{k}$-tuple, $(\bar{m}_1, ..., \bar{m}_{2^k})$ leads to a distinct tree of depth $k+1$, and there are $(m-1)^{2^k}$ of those. Hence, we have a bound $|\tilde{\mathcal{T}}^{(k+1, m)}| \geq (m-1)^{2^k} |\tilde{\mathcal{T}}^{(k, m)}|$, and therefore $|\tilde{\mathcal{T}}^{(k+1, m)}| \geq (m-1)^{\sum_{k'=1}^k 2^{k'}} = (m-1)^{2^{k+1} - 1}$.


% we assume that $i_1^{(k, m)}, ..., i_{2^k}^{(k, m)}$ all have distinct paths leading to them from the root node,  

\end{proof}
Thus, by counting the number of depth-$k$ rooted subtrees, we derive the following result:
\begin{proposition}
The total number of node equivalence classes among depth-$k$ egonets induced by WL-type GNNs is $\Omega(m^{(2^k)})$.
\end{proposition}

In comparison, we will next argue that the equivalence classes induced by Simplified GNNs are more coarsened. To see this, let's first consider the example where $\Omega = \{I, \tilde{A}, \tilde{A}^2, ...\}$, with $\tilde{A} = D^{-\alpha} A D^{-\beta}$ for any $\alpha, \beta \in \mathbb{R}$. Then
% \begin{equation}
%     \tilde{X}_t = \tilde{A}^t X = \left ( D^{-\alpha} A 
% \end{equation}
\begin{equation}
    \begin{split}
        (\tilde{X}_t)_i =& (\tilde{A}^t X)_i \\
        =& \sum_{(i, i_1, ..., i_t) \in \mathcal{W}_t(G, i)} d_i^{-\alpha} d_{i_1}^{-(\alpha + \beta)} \cdot ... \cdot d_{i_{t-1}}^{-(\alpha + \beta)} \cdot d_{i_{t}}^{-\beta} \cdot X_{i_t} \\
        =& d_i^{-\alpha} \cdot \sum_{\substack{(i, i_1, ..., i_t) \in \mathcal{W}_t(G, i), \\ \{ \{ d_{i_1}, ..., d_{i_{t-1}} \} \} = \{ \{ \bar{d}_1, ..., \bar{d}_{t-1} \} \} \\ d_{i_t} = \bar{d}_t \\ X_{i_t} = x}} (\bar{d}_1 \cdot ... \cdot \bar{d}_{t-1})^{-(\alpha + \beta)} \cdot \bar{d}_t \cdot x \\
        =& d_{i}^{-\alpha} \cdot \sum_{\{ \{ \bar{d}_1, ..., \bar{d}_{t-1} \} \}, \bar{d}_t, x} (\bar{d}_1 \cdot ... \cdot \bar{d}_{t-1})^{-(\alpha + \beta)} \cdot \bar{d}_t \cdot x \cdot |\mathcal{W}_t(G, i; \{ \{ \bar{d}_1, ..., \bar{d}_{t-1} \} \}, \bar{d}_t, x)|~,
    \end{split}
\end{equation}
where we define $\mathcal{W}_t(G, i)$
to be the set of walks of length $t$ in $G$ starting from node $i$, and $\mathcal{W}_t(G, i; \{ \{ \bar{d}_1, ..., \bar{d}_{t-1} \} \}, \bar{d}_t, x) \subseteq \mathcal{W}_t(G, i)$ to be the subset of them whose degree multiset ...
Hence, $(\tilde{X}_t)_i$ is completely characterized by the number of walks in each of these sets. Thus, to upper-bound the number of node equivalence classes induced by a Simplified GNN with such an $\Omega$, we can upper-bound the number of such sets for each operator $\tilde{A}^t$. This approach allows us to derive

\begin{proposition}
If $\Omega = \{ \tilde{A}, \tilde{A}^2, ...\}$, where $\tilde{A} = D^{-\alpha} A D^{-\beta}$ for any $\alpha, \beta \in \mathbb{R}$, then the total number of node equivalence classes among depth-$k$ egonets induced by the Simplified GNN is exponential in $k$.
\end{proposition}

\begin{proposition}
If $\Omega$ is any family of equivariant linear operators on the graph that only depends on the graph topology, then there exists a node equivalence class induced by a Simplified GNN with $\Omega$ that contains doubly-exponential-in-$k$ number of node equivalence classes induced by the family of WL-type GNNs.
\end{proposition}



% In particular, WL-type models like Message Passing Neural Networks (MPNNs) define functions on the rooted subtree of the target node. Formally, if we use $T^{(k)}(i, G)$ to denote the depth-$k$ subtree rooted at node $i$ in graph $G$, then an MPNN of $k$ layers maps $T^{(k)}(i, G)$ to the label it predicts for node $i$. It is not hard to see that
% \begin{proposition}
% The family of MPNNs of depth $k$, as node-wise functions, is able to approximate any function on the rooted subtree of depth $k$
% .
% \end{proposition}
% What about SWL-type models? Given a tree $T$ of depth at least $k$, let $L^{(k)}(T)$ denote the multi-set of the depth-$k$ leaf nodes of $T$. Then, let $S^{(k)}(T) = \{ X_i: i \in L^{(k)}(T)\}_m$ be the multi-set of the node features of all the depth-$k$ leaf nodes of $T$.
% % Let $L(T^{(k)}(i, G))$ denote the multi-set of leaf nodes of $T^{(k)}(i, G)$, or the depth-$k$ leaf node in the subtree rooted at $i$. Note that different leaf nodes of $T^{(k)}(i, G)$ may correspond to the same node in the original graph $G$. Then, let $S^{k}(i, G) = \{ X_i: i \in L(T^{(k)}(i, G))\}_m$ be the multi-set of the node features of all the leaf nodes of $T^{(k)}(i, G)$. 
% Then, we can see that
% \begin{proposition}
% \label{prop:swl_multisets}
% A function $f$ on the set of rooted subtrees of depth-$k$ can be approximated by SWL-type models if and only if $\forall$ tree $T$ of depth $k$, $f(T)$ can be expressed as $f(T) = g(S^{(0)}(T), ..., S^{(k)}(T))$ for some function $g$ on $(k+1)$-tuples of multi-sets.
% \end{proposition}

Having characterized the relative sizes and numbers of WL-type GNNs and Simplified GNNs as such, a next question is whether we can find explicitly some functions expressible by WL-type GNNs but not Simplified GNNs. Indeed, such functions exist. For example,
% \begin{proposition}
% For $k > 1$, for any path $\mathtt{P}$ of length $k$, the counting function of $\mathtt{P}$ on trees of depth $k$ can be approximated by WL-type models but not SWL-type models.
% \end{proposition}
% \begin{corollary}
% WL-type models of $k$ layers are able to count the number of any walks of length $k$, which can not be done with SWL-type models of any depth.
% \end{corollary}
for $k > 1$, a walk $\mathtt{W} = (i_1, ..., i_k)$ of length $k$ is characterized by the pair of $k$-tuples of the degrees and node features of the nodes on the walk, i.e. $(d_{i_1}, ..., d_{i_k})$ and $(X_{i_1}, ..., X_{i_k})$. We consider the functions that count the total number of walks starting from the root of the egonet that give rise to the same $k$-tuple of node features.
\begin{proposition}
For $k > 1$, for $k$-tuple of node features, $(x_1, ..., x_k)$, the function that counts the total number of walks starting from the root of the egonet that give rise to the this $k$-tuple of node features can be approximated by WL-type GNNs but not Simplified GNNs with any $\Omega$.
\end{proposition}
Having found a gap between WL-type models and SWL-type models in terms of representing functions on rooted subtrees, a key question still remains: is this gap relevant to real-world tasks?

% \section{Relevance of the Expressive Power Gap in Real Datasets}
% Here is a theoretical upper-bound on the performance of depth-$k$ SWL-type models on node-wise prediction tasks: 

% We define an equivalence relation among trees of depth-$k$ as follows. For two trees $T_1$ and $T_2$, both of depth-$k$, we consider them as equivalent (and write as $T_1 \simeq T_2$) if $\forall k' \leq k$, there is $S^{(k')}(T_1) = S^{(k')}(T_2)$.
% In a node-wise prediction task on $G = (V, E)$,  we define $\mathcal{T}^{(k)}(G) = \{ T^{(k)}(i, G): i \in V \}$ to be the set of all depth-$k$ rooted subtrees in $G$. It is partitioned by $\simeq$ into equivalence classes, which also induce a partition of the vertex set $V$ into equivalence classes. By Proposition~\ref{prop:swl_multisets}, we know that any SWL-type model will necessarily compute the same outcome when applied to any rooted subtree in a given equivalence class. Therefore, in a classification task, for example, where the target label is discrete, the best possible (Bayes-optimal) performance of any SWL-type model is to predict the mode of the labels of all the nodes in the corresponding equivalence class.

% We can actually try to compute this lower-bound on the error of SWL-type models on real datasets.

\section{Generalization}
% \subsection{Lower bound on the VC dimension of GNNs}
% Consider the case where node features are binary and all nodes have degree at most $m$. Let $\mathcal{T}^{(k, m)}$ be the space of all computation trees (rooted subtrees) of depth $k$ and degree at most $m$, in which each node has feature $0$ or $1$.
\begin{corollary}
The VC dimension of GNNs of $k$ layers (with no bound on weights) as functions on depth-$k$ egonets is $O(m^{(2^k)})$.
\end{corollary}
% \begin{lemma}
% $|\mathcal{T}^{(k, m)}| \geq (m-1)^{(2^{k}-1)}$.
% \end{lemma}
% \begin{proof}
% let $L^{(k)}(T)$ denote the set of the depth-$k$ leaf nodes of a tree $T$. There are $2^k$ paths of length $k$, from $(0, 0, ..., 0)$ to $(1, 1, ..., 1)$. We index them according to the dictionary order, with $\mathtt{P}^{(k)}_1 = (0, 0, ..., 0)$ and $\mathtt{P}^{(k)}_{2^k} = (1, 1, ..., 1)$.
% To lower-bound the cardinality of $\mathcal{T}^{(k, m)}$, we lower-bound the cardinality of its subset, $\tilde{\mathcal{T}}^{(k, m)}$, defined to be those computation trees in $\mathcal{T}^{(k, m)}$ which contain all $2^k$ possible paths of length $k$. This means that, for each $T \in \tilde{\mathcal{T}}^{(k, m)}$, $L^{(k)}(T) = \cup_{\tau = 1}^{2^k} S_{\tau}$, with each $S_{\tau}$ non-empty and satisfying that the path from the root node to every node in $S_{\tau}$ is exactly $\mathtt{P}^{(k)}_\tau$.

% % $\exists$ nodes $i_1^{(k, m)}, ..., i_{2^k}^{(k, m)}$ such that the paths from the root node to each of them are all distinct. 
% Next, we construct computation trees of depth $k+1$ by assigning children of feature $0$ or $1$ to the leaf nodes in $T$. First note that, with two distinct computation trees $T$ and $T' \in \tilde{\mathcal{T}}^{(k, m)}$, we obtain distinct computation trees in $\tilde{\mathcal{T}}^{(k+1, m)}$ in this way. There are obviously many choices to assign the children. To get a lower-bound on the cardinality of $\tilde{\mathcal{T}}^{(k+1, m)}$, we only need to consider a subset of these choices of assignments, namely, those that assign the same number of children with feature $1$ to nodes in the same $S_{\tau}$.
% Thus, we let $\bar{m}_\tau$ denote the number of children of feature $1$ assigned to the nodes in $S_\tau$. Due to the constraint that each node in the computation subtree must have its parent's feature as one of its children's feature, not all choices of $\{ \bar{m}_\tau \}_{\tau=1}^{2^k}$ lead to legitimate computation trees. Nonetheless, when restricting to the cases where $\forall \tau \in [2^k], 1 \leq \bar{m}_{\tau} \leq m-1$, we see that every node in $L^{(k)}(T)$ has at least one child of feature $0$ and another child of feature $1$, thereby satisfying the constraint whether its parent has feature $0$ or $1$. Moreover, because of this, the new tree of depth $k+1$ obtained in this way contains all $2^{k+1}$ possible paths of length $k+1$, and therefore belongs to $\tilde{\mathcal{T}}^{(k+1, m)}$. Hence, what is left to do is to show a lower bound on how many such trees in $\tilde{\mathcal{T}}^{(k+1, m)}$ can be obtained from each $T$. Because nodes in $S_\tau$ are distinguishable from nodes in $S_{\tau'}$ for $\tau \neq \tau'$, we see that every choice of the $2^{k}$-tuple, $(\bar{m}_1, ..., \bar{m}_{2^k})$ leads to a distinct tree of depth $k+1$, and there are $(m-1)^{2^k}$ of those. Hence, we have a bound $|\tilde{\mathcal{T}}^{(k+1, m)}| \geq (m-1)^{2^k} |\tilde{\mathcal{T}}^{(k, m)}|$, and therefore $|\tilde{\mathcal{T}}^{(k+1, m)}| \geq (m-1)^{\sum_{k'=1}^k 2^{k'}} = (m-1)^{2^{k+1} - 1}$.


% % we assume that $i_1^{(k, m)}, ..., i_{2^k}^{(k, m)}$ all have distinct paths leading to them from the root node,  

% \end{proof}
% This a consequence of the fact that GNNs of $k$ layers are able to approximate arbitrary functions on trees.

\begin{corollary}
The VC dimension of Simplified GNNs with $\Omega = \{ \tilde{A}, \tilde{A}^2, ..., \tilde{A}^k \}$, where $\tilde{A} = D^{-\alpha} A D^{-\beta}$ for any $\alpha, \beta \in \mathbb{R}$ as functions on depth-$k$ egonets is at most exponential-of-polynomial-in-$k$.
\end{corollary}



\bibliography{ref}
\bibliographystyle{plain}


\end{document}



==> summary_08312020.tex <==
% \documentclass{article}
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{natbib}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{graphicx}

% \title{multi-hop vs depth}
% \author{zc1216 }
% \date{August 2020}

\begin{document}


Consider graph-level predictions on graphs without edge features. Two classical models are
\begin{itemize}
\item GCN of T layers:\\
$H^{0} = X^{0}$.
Then, for $t \in \{0, …, T-1\}$,
\begin{equation}
    H^{(t+1)} = \sigma(D^{-1/2} A D^{-1/2} H^{(t)} W^{(t)})
\end{equation}
Then $H^{(out)} = H^{(T)}$ for node-level outputs.

\item “Regular GNN” of T layers:\\
$H^{0} = X^{0}$. Then, for $t \in \{0, …, T-1\}$,
\begin{equation}
    H^{(t+1)} = \sigma(A H^{(t)} W^{(t)})
\end{equation}
Then $H^{(out)} = H^{(T)}$ for node-level outputs.
\end{itemize}
Their expressive power in terms of graph isomorphism testing is upper-bounded by the WL test:
\begin{itemize}
\item WL test of T iterations: \\
For $t \in \{0, …, T-1\}$,
\begin{align}
    \tilde{c}^{t}(i) =& \cup_{j \in N_1(i)} \{\{ c^{t}(j) \}\} \\
    c^{t+1}(i) =& (c^{t}(i), \tilde{c}^{t}(i))
\end{align}
Finally $c^{out}(i) = c^{T}(i)$.
\end{itemize}


There have been several attempts to simplify these models by using families of multi-hop operators to replace the role of depth in GNNs (in additino to our model for community detection). Such models belong to the following framework:

\paragraph{Multi-hop Shallow GNNs:}
Let $\Omega(A) = \{ \omega_1(A)$, ..., $\omega_T(A) \}$ be a set of (usually multi-hop) operators that are functions of the adjacency matrix, $A$. We first apply each of these operators (on the left) to input node features $X \in \mathbb{R}^{n \times d_0}$ and concatenate the output vectors (along a third dimension) into a tensor $Z \in \mathbb{R}^{n \times d_0 \times T}$:
\begin{equation}
    Z = \big | \big |_{t=1}^T \omega_t(A) X
\end{equation}
which means
\begin{equation}
    Z_{:, :, t} = \omega_t(A) X
\end{equation}
We then apply a certain node-wise function $\rho: \mathbb{R}^{n \times d_0 \times T} \to \mathbb{R}^{n \times d'}$ on H and finally a pooling function $\phi: \mathbb{R}^{n \times d'} \to \mathbb{R}$, obtaining
\begin{equation}
    \hat{Y} = \phi(\rho(H)) \in \mathbb{R}
\end{equation}


Here are some examples:
\begin{itemize}
    \item Simple Graph Convolution \cite{wu2020simplifying}:\\
    $\Omega(A) = \{ (\tilde{D}^{-1/2} \tilde{A} \tilde{D}^{-1/2})^T \}$ for some $T > 0$, with $\tilde{A} = A + I$ and $\tilde{D}$ being the degree matrix of $\tilde{A}$; 
    % $\sigma$ being the softmax function.
    $\rho(H) = softmax(H W)$. Thus,
    \begin{equation}
        \hat{Y} = \phi(softmax((\tilde{D}^{-1/2} \tilde{A} \tilde{D}^{-1/2})^T X W))
    \end{equation}
    
    \item Graph Feature Network \cite{chen2019powerful}:\\
    $\Omega(A) = \{ I, D, \omega_1(A)$, ..., $\omega_T(A) \}$, with $\omega_t(A) = (\tilde{D}^{-1/2} (A + \epsilon I) \tilde{D}^{-1/2})^t$; $\rho$ is an MLP applied to the vectorization of $Z_{i, :, :} \in \mathbb{R}^{T \times d_0}$ for each node $i$; $\phi$ is also an MLP.
    
    \item Scalable Inception Graph Networks \cite{rossi2020sign}:\\
    $\Omega(A) = \Omega_1(A) \cup \Omega_2(A) \cup \Omega_3(A)$, where $\Omega_1(A)$ is a family of simple / normalized adjacency matrices, $\Omega_2(A)$ is a family of Personalized-PageRank-based adjacency matrices, and $\Omega_3(A)$ is a family of ``triangle-based" adjacency matrices; $\rho: \mathbb{R}^{n \times d_0 \times T} \to \mathbb{R}^{n \times Td_1}$, defined to be 
    $\rho(Z)_{:, :, (t-1)d_1:td_1} = \sigma_2(\sigma_1(Z_{:, :, t} W_t)W_{out})$ with each $W_t \in \mathbb{R}^{d_0 \times d_1}$ and $W_{out} \in \mathbb{R}^{T d_1 \to d'}$.
    
\end{itemize}

Our goal is to study the expressive power of this type of models, especially compared to WL / the regular GNNs. We first focus on two specific choices of $\Omega(A)$:
\begin{itemize}
\item Simplified-GNN-1 of T-hop neighborhood:\\
% $H^{0} = X^{0}$. Then,
% \begin{equation}
%     H^{out} = \sigma(\sum_{t=1}^T A^{(t)} H^{(0)} W^{(t)})
% \end{equation}
$\Omega(A) = \{ I, A, ..., A^T \}$.

\item Simplified-GNN-2 of T-hop neighborhood:\\
% $H^{0} = X^{0}$. Then,
% \begin{equation}
%     H^{out} = \sigma(\sum_{t=1}^T A^{(t)} H^{(0)} W^{(t)})
% \end{equation}
$\Omega(A) = \{ I, \min(A, 1), ..., \min(A^T, 1) \}$

% \item Simplified-GNN-3 of T-hop neighborhood:

\end{itemize}

We want to first show that their expressive power in terms of graph isomorphism testing corresponds to the two following WL-like tests:

\begin{itemize}

\item Simplified-WL-1 of T iterations:\\
Define $w_t(i, j)$ to be the number of walks (allowing backtracking) of length t from $i$ to $j$.\\ 
For $t \in \{1, …, T\}$,
\begin{align}
    \tilde{c}^{t}(i) =& \cup_{count \leq w_t(i, j)} \{\{ c^{0}(j) \}\}_{j \in N_1(i)} \\
c^{out}(i) =& (c^{0}(i), \tilde{c}^{1}(i), …, \tilde{c}^{T}(i))
\end{align}

\item Simplified-WL-2 of T iterations:\\
For $t \in \{1, …, T\}$,
\begin{align}
    \tilde{c}^{t}(i) =& \cup_{j \in N_t(i)} \{\{ c^{0}(j) \}\} \\
c^{out}(i) =&(c^{0}(i)), \tilde{c}^{1}(i), …, \tilde{c}^{T}(i))
\end{align}

\item Simplified-WL-3 of T iterations:\\
\begin{equation}
c^{out}(i) = (c^{0}(i)), \cup_{j \in \cup_{t=1}^T N_t(i)} \{\{ (c^{0}(j), w_1(i, j), …, w_t(i, j) ) \}\} )
\end{equation}
\end{itemize}

In particular, on graphs without node features, we have
\begin{itemize}
    \item Simplified-WL-1 of T iterations becomes:
\begin{equation}
    c^{out}(i) = (w_1(i), …, w_T(i))
\end{equation}

\item Simplified-WL-2 of T iterations becomes:
Define $d_t(i)$ to be the size of the t-hop neighborhood of $i$. Then
\begin{equation}
    c^{out}(i) = (d_1(i), …, d_T(i))
\end{equation}

\end{itemize}

We will then try to study the power of these simplified-WL tests. In particular, we have found that
\begin{enumerate}
    \item There exist pairs of graphs that can be distinguished by WL and Simplified-WL-2 but not Simplified-WL-1 
    \begin{figure}[h]
        \centering
        \includegraphics[scale=0.08]{SWL-1 counter.jpg}
        % \caption{Caption}
        \label{fig:my_label}
    \end{figure}
    
    \item There exists pairs of graphs that can be distinguished by Simplified-WL-2 but not WL or Simplified-WL-1:\\
    Two triangles v.s. one hexagon (in fact, SWL-2 can count triangles)
    
    \item There exists pairs of graphs that can be distinguished by $2$ iterations of WL or Simplified-WL-1 but not $2$ iterations of Simplified-WL-2.
    
    \item SWL-1 and SWL-2 should be no more powerful than 2-WL.
\end{enumerate}

\paragraph{Further Questions:}
\begin{enumerate}
    \item Can we found counterexamples to SWL-2 for arbitrary number of iterations?
    \item How general or common are the counterexamples to SWL-1?
    \item How does SWL-(1+2) compare with WL?
    \item The effect of spatial batchnorm
    \item How to relate to node-level tasks?
\end{enumerate}

\bibliography{ref}
\bibliographystyle{plain}


\end{document}
